Voter-like dynamics with conflicting preferences on modular networks

Two of the main factors shaping an individual's opinion are social coordination and personal preferences, or personal biases. To understand the role of those and that of the topology of the network of interactions, we study an extension of the voter model proposed by Masuda and Redner (2011), where the agents are divided into two populations with opposite preferences. We consider a modular graph with two communities that reflect the bias assignment, modeling the phenomenon of epistemic bubbles. We analyze the models by approximate analytical methods and by simulations. Depending on the network and the biases' strengths, the system can either reach a consensus or a polarized state, in which the two populations stabilize to different average opinions. The modular structure has generally the effect of increasing both the degree of polarization and its range in the space of parameters. When the difference in the bias strengths between the populations is large, the success of the very committed group in imposing its preferred opinion onto the other one depends largely on the level of segregation of the latter population, while the dependency on the topological structure of the former is negligible. We compare the simple mean-field approach with the pair approximation and test the goodness of the mean-field predictions on a real network.

==> 0_Abstract.tex <==
\begin{abstract}
Two of the main factors shaping an individual's opinion are social pressure and personal preference.
% , that may drive a system of interacting individuals towards the convergence to a polarized state.
% When these two happen to be in contrast, people can either behave in dissonance with their personal believes in order to favour social consensus or, when their bias is dominant, persist in their preferred opinion and accept conflict more easily. 
We study an extension of the voter model proposed by Masuda and Redner (2011), where the interacting agents are divided into two populations with opposite external biases of different intensities. We analyze the role of the underlying social network, considering a modular graph with two communities that reflect the bias assignment, modeling the phenomenon of epistemic bubbles (Nguyen, 2020). Depending on the network and the biases' strengths, the system can either reach a consensus (common agreement, zero polarization) or a polarized state, in which the two populations stabilize to different average opinions. It turns out that generally the modular structure has the effect of increasing both the value of the polarization and the size of the polarization region in the space of parameters. We also show that, when the discrepancy in bias between the populations is high, the success of the very committed one in imposing its preferred opinion depends largely on the level of segregation of the other population, while the dependency on its own topological structure is negligible. We compare the mean-field dynamics with the one deriving from the Pair approximation and test the goodness of the mean-field predictions on a real network.
\end{abstract}

==> Not in the file/Annealed_approximation.tex <==
\section{Annealing approximation}
We rewrite the dynamical system in terms of the total density of up spin $\rho$ and the polarization $\Delta$, defined as
\begin{align*}
&\rho = \rho_1 + \rho_2 \\
&\Delta = \frac{\rho_1}{\alpha} - \frac{\rho_2}{1-\alpha}    
\end{align*}
Substituing those in the system (\ref{fc mf rho12}), we get
\begin{equation}
    \begin{cases}
        \dot{\rho} = [\alpha h_1 +(1-\alpha)h_2]\rho(1-\rho) - \Delta\alpha(1-\alpha)(h_1-h_2)(\rho-\frac{1}{2}) \\
        \dot{\Delta} = (h_1-h_2)\rho(1-\rho) - \Delta\bigg[[(1-\alpha)h_1+\alpha h_2](\rho-\frac{1}{2}) + \frac{1}{2}\bigg]
    \end{cases}
\label{fc rhodelta}
\end{equation}
The "annealing" approximation consists in assuming that there is no distinction, on average, between the magnetizations of two classes, in other words that $\Delta(t)\approx0$ at all times. \\
Within the annealing approximation, the evolution equation is single (only on the density $\rho$) and becomes
\begin{equation}
    \dot{\rho} = [\alpha h_1 +(1-\alpha)h_2]\rho(1-\rho)
\end{equation}
defining the "effective bias"
\begin{equation}
    H = \alpha h_1 +(1-\alpha)h_2
\end{equation}
we get 
\begin{equation}
    \frac{d\rho}{dt} = H\rho(1-\rho)
\end{equation}
Indeed another way to interpret the annealed setting is to assume that the features of the classes, in this model the biases, are random variable extracted at every iteration with a probability correspondent to their density in the system, i.e. at each iteration each node has bias $h_1$ with probability $\alpha$ and $h_2$ with probability $1-\alpha$.\\
The annealing approximation is applied but uncontrolled in \cite{}. To control it, we can derive an upper bound on $\Delta(t)$, namely $\Delta_{max}$, and assuming that as long as $\Delta_{max}$ is small, the annealing approximation $\Delta(t)\simeq 0\;\forall t$ works well. Eventually, we test this assumption by comparing with numerical simulations. Notice that since by hypothesis $h_1\geq 0$ and $h_2\leq0$, and starting from a randomic initial distribution of the opinions, $<\Delta>(t)$ is always non-negative and thus there is no need to set a lower bound.\\
We have defined $\Delta_{max}$ as the maximum value reachable by $\Delta$, i.e. the value over which $\Delta$ is systematically pushed back towords zero ($\dot{\Delta}<0$). Looking at the second equation of (\ref{fc rhodelta}), since the first term is always positive and so is the term multiplying $\Delta$, we get that
\begin{equation}
    \Delta_{max} = max_{\rho\in[0,1]} \frac{A\rho(1-\rho)}{B(\rho-\frac{1}{2})+\frac{1}{2}}
\end{equation}
with $A=h_1-h_2$ and $B=(1-\alpha)h_1+\alpha h_2$.\\
The latter maximization is satisfied by 
\begin{equation}
    \rho^* \equiv argmax_{\rho\in[0,1]}  \frac{A\rho(1-\rho)}{B(\rho-\frac{1}{2})+\frac{1}{2}} = \frac{1}{2} \bigg(1-\frac{1-\sqrt{1-B^2}}{B}\bigg)
\end{equation}
Notice that $\rho^*\in[0,1]$ is satisfied ($|B|\leq1$ always), and $\rho^*<\frac{1}{2}$ if $B>0$, viceversa $\rho^*>\frac{1}{2}$ if $B<0$, eventually $\rho^*=\frac{1}{2}$ if $B=0$.\\
Substituting back, we have that
\begin{equation}
    \Delta_{max} = (h_1-h_2) \frac{1-\sqrt{1-B^2}}{B^2}
\end{equation}
Notice that $\Delta_{max}\geq\frac{h_1-h_2}{2}$, and expanding for small $B$ we have that $\Delta_{max} = \frac{h_1-h_2}{2} +O(B^2)$.
\\
\\
The single evolution equation derived by the annealing approximation is solvable and the solution, i.e. the evolution of the density of up spins starting from an initial density $\rho_0$, reads 
\begin{equation}
    \rho(t) = \frac{1}{1+(\frac{1-\rho_0}{\rho_0})e^{-Ht}}
\end{equation}
which for uniformly random initial conditions ($\rho_0=0$) is simply
\begin{equation}
    \rho(t) = \frac{1}{1+e^{-Ht}}
\end{equation}
Indeed the annealed approximation is equivalent to the single population biased voter model with effective bias $H$, which always predicts the approach to consensus as long as $H\neq 0$.\\
\\
Within the annealing approximation, it is possible to calculate the exit probability $E(\rho)$, i.e. the probability to reach positive consensus in a finite system (an infinite system it always approaches consensus) as a function of the initial density of up spins. Following \cite{}, one writes the Backward-Kolmogorov equation for the exit probability
\begin{equation}
    E(\rho) = R^+(\rho)E(\rho+\delta\rho)+R^-(\rho)E(\rho-\delta\rho) +[1-R^+(\rho)-R^-(\rho)]E(\rho)
\end{equation}
with $\Delta\rho = \frac{1}{N}$, and boundary conditions $E(1)=1,E(0)=0$. The global transition rates are considered in the annealed setting:
\begin{align*}
    \begin{cases} 
    R^{+}(\rho) = (1-\rho)\bigg(\alpha\frac{1+h_1}{2} + (1-\alpha)\frac{1+h_2}{2}\bigg)\rho = (1-\rho)\frac{1+H}{2}\rho \\
    R^{-}(\rho) = \rho\bigg(\alpha\frac{1-h_1}{2} + (1-\alpha)\frac{1-h_2}{2}\bigg)(1-\rho) = \rho\frac{1-H}{2}(1-\rho)\\
    \end{cases}
\end{align*}
Using $\rho = \frac{n}{N}$, the equation becomes
\begin{equation}
    E(n) = \frac{1+H}{2}E(n+1)+\frac{1-H}{2}E(n-1) 
\end{equation}
whose solution satisfying boundary conditions is 
\begin{equation}
    E(n) = \frac{1-(\frac{1-H}{1+H})^n}{1-(\frac{1-H}{1+H})^N}
\end{equation}
and thus substituting back the density
\begin{equation}
    E(\rho) = \frac{1-(\frac{1-H}{1+H})^{\rho N}}{1-(\frac{1-H}{1+H})^N}
\end{equation}
Starting from uniformly random initial conditions, the expression above becomes
\begin{equation}
    E(\small\frac{1}{2}) = \frac{1}{1+(\frac{1-H}{1+H})^{\frac{N}{2}}}
\label{exit_homo}
\end{equation}
In figure \ref{}, we check test the validity of (\ref{exit_homo}) for multiple values of $\alpha$ in a small system $N=50$, comparing numerical estimations with the analytical predictions. In both the figures we fix the value of $h_2$ and represent the analytical prediction and the empirical simulations of the exit probability varying the first population's bias $h_1$. In the first figure we set $h_2=0$, which corresponds to the biased vs unbiased case studied in \ref{}, while in the second $h_2=-0.1$. The results confirm the validity of the assumption at the root of the annealing approximation: when $\Delta_{max}$ is low (i.e. when $h_1$ is low, see subfigure), the values of the exit probability predicted within the annealing approximation match with the empirical ones. For larger values of $\Delta_{max}$, instead, the predictions are far from being correct.\\

% We see that in general the prediction of the exit probability calculated within the anneanling apporximation is good for low $\Delta_{max}$, which correspond for both cases to small $h_1$. However, for $h_2=-0.1$ $\Delta_{max}$ is larger for small $h_1$ and thus it turns out that the approximation loses in accuracy before,increasing $h_1$, with respect to the $h_2=0$ case.
\\
% One could also derive and test a prediction on the mean time to reach consensus, within the annealing approximation.

\begin{figure}
\subfloat{\includegraphics[width = 0.5\textwidth]{Figures/exitproba1.png}} 
\subfloat{\includegraphics[width = 0.5\textwidth]{Figures/exitproba2.png}}\\
\subfloat{\includegraphics[width = 0.5\textwidth]{Figures/deltamax1.png} }
\subfloat{\includegraphics[width = 0.5\textwidth]{Figures/deltamax2.png}} \\ \\
\caption{\textbf{Annealing approximation.} \textit{Upper plots}: numerical simulations (triangles) and analytical predictions (lines) of the exit probability at $\rho = \frac{1}{2}$ of a system with $N=50$ agents, fixing $h_2 = 0$ (left) and $h_2 = -0.1$ (right), for different fractions of agents of the first populations $\alpha$ (colors), as function of the first population's bias $h_1$. \textit{Lower plots}: value of the quantity that controls the validity of the annealing approximation $\Delta_{max}$ as a function of $h_1$, obtained from equation \ref{}, respectively for $h_2 = 0$ (left) and $h_2 = -0.1$ (right). In order to calculate numerically the exit probability, we performed $10000$ runs of the model and iterated until convergence, thus we took the fraction of runs that reached the up consensus state.}
\label{fig:annealing}
\end{figure}


==> Not in the file/Echochamber.tex <==
\subsection{Echochambers: fixing the average internal and external degrees}
To study the BVM on the SBM we choose to fix the average internal and external degrees. The mean field equations depend on the fixed average degrees only through
\begin{align*}
    &\gamma_1 = \frac{z_{12}}{z_{11}+z_{12}}\\
    &\gamma_2 = \frac{z_{21}}{z_{22}+z_{21}}
\end{align*}
are the fractions of external links over the degree of the nodes of respectively the first and second community, and are called the "open-mindedness" of individuals of community 1 and 2. Note that $\gamma_1 = \frac{p_{12}(1-\alpha)}{p_{11}\alpha +p_{12}(1-\alpha)}$ and $\gamma_2 = \frac{p_{21}\alpha}{p_{22}(1-\alpha) +p_{21}\alpha}$.\\
\\
Defining the normalized dynamical variables $\rho'_1 = \frac{\rho_1}{\alpha} \in [0,1]$, $\rho'_2 = \frac{\rho_2}{1-\alpha} \in [0,1]$
\begin{equation}
\begin{cases}
    \dot{\rho'_1} = \frac{1}{2}\bigg[   (1-\rho'_1)(1+h_1)[(1-\gamma_1)\rho'_1+\gamma_1\rho'_2] - \rho_1(1-h_1)[(1-\gamma_1)(1-\rho'_1)+\gamma_1(1-\rho'_2)]\bigg]  \\
    \dot{\rho'_2} = \frac{1}{2}\bigg[ (1-\rho'_2)(1+h_2)[\gamma_2\rho'_1+(1-\gamma_2)\rho'_2) - \rho'_2(1-h_2)[\gamma_2(1-\rho'_1)+(1-\gamma_2)(1-\rho'_2)] \bigg] 
\end{cases}
\label{mf_echochambers}
\end{equation}


\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{Figures/echochamb_final_good.png}
    \caption{\textbf{Biased Voter Model on echochambers.} Mean-field predictions for the polarization (eq. \ref{mf_echochambers}) in the $h_1h_2$ plane for two equally "open-minded" echochambers ($\gamma_1=\gamma_2$), varying the open-mindedness parameter. Decreasing the open-mindedness, the consensus areas shrink and the system becomes more and more polarized.}
    \label{fig:echo_equal gamma}
\end{figure}
